Unveiling the Ambiguity in Neural Inverse Rendering: A Parameter Compensation Analysis

Inverse rendering aims to reconstruct the scene properties of objects solely from multiview images. However, it is an ill-posed problem prone to producing ambiguous estimations deviating from physically accurate representations. In this paper, we utilize Neural Microfacet Fields (NMF), a state-of-the-art neural inverse rendering method to illustrate the inherent ambiguity. We propose an evaluation framework to assess the degree of compensation or interaction between the estimated scene properties, aiming to explore the mechanisms behind this ill-posed problem and potential mitigation strategies. Specifically, we introduce artificial perturbations to one scene property and examine how adjusting another property can compensate for these perturbations. To facilitate such experiments, we introduce a disentangled NMF where material properties are independent. The experimental findings underscore the intrinsic ambiguity present in neural inverse rendering and highlight the importance of providing additional guidance through geometry, material, and illumination priors.

==> sec/apendix_backup.tex <==
% \newpage
\clearpage
\section{Results per Scene}
In this section, we present additional results from our experiments regarding the interactions and compensations between scene properties. \cref{fig:interactions:all} presents the examined metrics PSNR, SSIM, LPIPS, MAE, and EPSNR for the ball, car, and helmet scenes of the shiny-blender dataset. Furthermore, we also provide the qualitative visualizations of these experiments for the ball (\cref{fig:finetune-image-grid-ball}) and helmet scenes (\cref{fig:finetune-image-grid-helmet}).\\

% FINE-TUNING RESULTS
\noindent\begin{minipage}{\textwidth}
    \centering
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/ball_finetuning_PSNR.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/ball_finetuning_SSIM.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/ball_finetuning_LPIPS.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/ball_finetuning_MAE.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/ball_finetuning_EPSNR.png}\\
    (a) ball
    %
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/car_finetuning_PSNR.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/car_finetuning_SSIM.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/car_finetuning_LPIPS.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/car_finetuning_MAE.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/car_finetuning_EPSNR.png}\\
    %
    (b) car
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/helmet_finetuning_PSNR.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/helmet_finetuning_SSIM.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/helmet_finetuning_LPIPS.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/helmet_finetuning_MAE.png}%
    \includegraphics[trim=40 40 0 0,clip,width=0.2\linewidth]{figures/exp2_metrics/helmet_finetuning_EPSNR.png}\\
    (c) helmet
    \captionof{figure}{Graphs demonstrating how one scene property can compensate for suboptimal estimation of other properties. The vertical axis corresponds to the manipulated scene property while the horizontal axis corresponds to the fine-tuned property. The arrows $\uparrow, \downarrow$ on the manipulated property labels refer to overestimating or underestimating the property, respectively. The arrows $\uparrow, \downarrow$ next to the metrics on the title of each plot, correspond with "higher is better" and "lower is better" respectively. The colormap is adapted so that lighter denotes better across all metrics. }
    \label{fig:interactions:all}
\end{minipage}

\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FINETUNING IMAGE GRID FOR BALL
\begin{figure*}[h]
    \centering
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{c c c c c c c c}
        & Manip. Property & \multicolumn{5}{c}{Fine-tuned Scene Property} \\[10pt]
        & & Albedo & Roughness & $\mathit{F_0}$ & Density & Env. Map \\
        \vspace{-0.35cm}
        % ALBEDO UNDER NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Albedo$\downarrow$}}} & 
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_albedo_noise_under.png}
            \put(-20,62){\small{38.49}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_albedo_albedo_under.png}
            \put(-20,62){\small{38.41}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_albedo_roughness_under.png}
            \put(-20,62){\small{38.41}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_albedo_f0_under.png}
            \put(-20,62){\small{38.42}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_albedo_density_under.png}
            \put(-20,62){\small{36.16}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_albedo_envmap_under.png}
            \put(-20,62){\small{38.36}}
        \end{subfigure}\\
        \vspace{-0.35cm}
        % ALBEDO OVER NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Albedo$\uparrow$}}} & 
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_albedo_noise_over.png}
            \put(-20,62){\small{30.53}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_albedo_albedo_over.png}
            \put(-20,62){\small{38.41}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_albedo_roughness_over.png}
            \put(-20,62){\small{38.43}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_albedo_f0_over.png}
            \put(-20,62){\small{38.43}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_albedo_density_over.png}
            \put(-20,62){\small{36.00}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_albedo_envmap_over.png}
            \put(-20,62){\small{38.36}}
        \end{subfigure}\\
        \vspace{-0.35cm}
        
        % ROUGHNESS UNDER NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Rough.$\downarrow$}}} & 
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_roughness_noise_under.png}
            \put(-20,62){\small{29.40}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_roughness_albedo_under.png}
            \put(-20,62){\small{35.09}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_roughness_roughness_under.png}
            \put(-20,62){\small{35.68}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_roughness_f0_under.png}
            \put(-20,62){\small{35.11}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_roughness_density_under.png}
            \put(-20,62){\small{33.64}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_roughness_envmap_under.png}
            \put(-20,62){\small{35.46}}
        \end{subfigure}\\
        \vspace{-0.35cm}

         % ROUGHNESS OVER NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Rough.$\uparrow$}}} & 
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_roughness_noise_over.png}
            \put(-20,62){\small{31.87}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_roughness_albedo_over.png}
            \put(-20,62){\small{33.66}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_roughness_roughness_over.png}
            \put(-20,62){\small{36.70}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_roughness_f0_over.png}
            \put(-20,62){\small{36.67}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_roughness_density_over.png}
            \put(-20,62){\small{35.06}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_roughness_envmap_over.png}
            \put(-20,62){\small{38.11}}
        \end{subfigure}\\
        \vspace{-0.35cm}
        
        % F0 UNDER NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{$\mathit{F_0}\downarrow$}}} & 
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_f0_noise_under.png}
            \put(-20,62){\small{28.69}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_f0_albedo_under.png}
            \put(-20,62){\small{38.37}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_f0_roughness_under.png}
            \put(-20,62){\small{38.38}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_f0_f0_under.png}
            \put(-20,62){\small{38.43}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_f0_density_under.png}
            \put(-20,62){\small{36.08}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_f0_envmap_under.png}
            \put(-20,62){\small{38.29}}
        \end{subfigure}\\
        \vspace{-0.35cm}
        
        % F0 OVER NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{$\mathit{F_0}\uparrow$}}} & 
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_f0_noise_over.png}
            \put(-20,62){\small{30.79}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_f0_albedo_over.png}
            \put(-20,62){\small{38.41}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_f0_roughness_over.png}
            \put(-20,62){\small{38.42}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_f0_f0_over.png}
            \put(-20,62){\small{38.42}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_f0_density_over.png}
            \put(-20,62){\small{36.19}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball_over/ball_f0_envmap_over.png}
            \put(-20,62){\small{38.34}}
        \end{subfigure}\\
        \vspace{-0.35cm}

        % DENSITY NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Density}}} & 
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_density_noise.png}
            \put(-20,62){\small{29.05}}
        \end{subfigure} &        
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_density_albedo.png}
            \put(-20,62){\small{29.17}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_density_roughness.png}
            \put(-20,62){\small{29.25}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_density_f0.png}
            \put(-20,62){\small{29.25}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_density_density.png}
            \put(-20,62){\small{36.13}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_density_envmap.png}
            \put(-20,62){\small{29.21}}
        \end{subfigure}\\
        \vspace{-0.35cm}
        
        % ENVMAP NOISE
        % 19.88	21.43	21.43	21.43	21.25	38.38
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Env. Map}}} & 
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_envmap_noise.png}
            \put(-20,62){\small{19.88}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_envmap_albedo.png}
            \put(-20,62){\small{21.43}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_envmap_roughness.png}
            \put(-20,62){\small{21.43}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_envmap_f0.png}
            \put(-20,62){\small{21.43}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_envmap_density.png}
            \put(-20,62){\small{21.25}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_envmap_envmap.png}
            \put(-20,62){\small{38.38}}
        \end{subfigure}\\[0.15cm]
        \hline \\[-0.3cm]
        
        % LEARNT PARAMS
        \multicolumn{2}{c}{Original Properties}
        \put(-75,-10){\small{PSNR $\rightarrow$ 38.44}} &
        \begin{subfigure}[c]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[c]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[c]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_f0.png}
        \end{subfigure} &
        \begin{subfigure}[c]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_density.png}
        \end{subfigure} &
        \begin{subfigure}[c]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -50 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_ball/ball_envmap.png}
        \end{subfigure}
    \end{tabular}
    % \vspace{1cm}
    \caption{Effect of manipulating one scene property before fine-tuning another for the helmet scene of the shiny-blender dataset \cite{verbin2022refnerf}. The arrows $\downarrow, \uparrow$ next to albedo, roughness, and $F_0$ denote underestimation or overestimation respectively. The bottom row contains the original properties before adding noise and fine-tuning. For every experiment, we also include the PSNR at the top right corner of the corresponding image.}
    \label{fig:finetune-image-grid-ball}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FINETUNING IMAGE GRID FOR HELMET
\begin{figure*}[h]
    \centering
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{c c c c c c c c}
        & Manip. Property & \multicolumn{5}{c}{Fine-tuned Scene Property} \\[10pt]
        & & Albedo & Roughness & $\mathit{F_0}$ & Density & Env. Map \\
        \vspace{-0.5cm}
        % ALBEDO UNDER NOISE
        % 24.95	30.93	30.92	30.92	29.96	33.44
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Albedo$\downarrow$}}} & 
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_albedo_noise_under.png}
            \put(-18,60){\small{24.95}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_albedo_albedo_under.png}
            \put(-18,60){\small{30.93}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_albedo_roughness_under.png}
            \put(-18,60){\small{30.92}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_albedo_f0_under.png}
            \put(-18,60){\small{30.92}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_albedo_density_under.png}
            \put(-18,60){\small{29.96}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_albedo_envmap_under.png}
            \put(-22,60){\small{33.44}}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % ALBEDO OVER NOISE
        % 26.12	33.37	33.32	33.31	31.72	33.36
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Albedo$\uparrow$}}} & 
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_albedo_noise_over.png}
            \put(-18,60){\small{26.12}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_albedo_albedo_over.png}
            \put(-18,60){\small{33.37}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_albedo_roughness_over.png}
            \put(-18,60){\small{33.32}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_albedo_f0_over.png}
            \put(-18,60){\small{33.31}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_albedo_density_over.png}
            \put(-18,60){\small{31.72}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_albedo_envmap_over.png}
            \put(-22,60){\small{33.36}}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % ROUGHNESS UNDER NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Rough.$\downarrow$}}} & 
        % 28.86	29.79	29.59	29.61	23.25	32.05
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_roughness_noise_under.png}
            \put(-18,60){\small{28.86}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_roughness_albedo_under.png}
            \put(-18,60){\small{29.79}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_roughness_roughness_under.png}
            \put(-18,60){\small{29.59}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_roughness_f0_under.png}
            \put(-18,60){\small{29.61}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_roughness_density_under.png}
            \put(-18,60){\small{23.25}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_roughness_envmap_under.png}
            \put(-22,60){\small{32.05}}
        \end{subfigure}\\
        \vspace{-0.5cm}

         % ROUGHNESS OVER NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Rough.$\uparrow$}}} & 
        % 25.34	27.39	27.45	27.4	27.07	28.09
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_roughness_noise_over.png}
            \put(-18,60){\small{25.34}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_roughness_albedo_over.png}
            \put(-18,60){\small{27.39}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_roughness_roughness_over.png}
            \put(-18,60){\small{27.45}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_roughness_f0_over.png}
            \put(-18,60){\small{27.40}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_roughness_density_over.png}
            \put(-18,60){\small{27.07}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_roughness_envmap_over.png}
            \put(-22,60){\small{28.09}}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % F0 UNDER NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{$\mathit{F_0}\downarrow$}}} & 
        % 25.82	33.43	33.41	33.48	29.61	33.49
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_f0_noise_under.png}
            \put(-18,60){\small{25.82}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_f0_albedo_under.png}
            \put(-18,60){\small{33.43}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_f0_roughness_under.png}
            \put(-18,60){\small{33.41}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_f0_f0_under.png}
            \put(-18,60){\small{33.48}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_f0_density_under.png}
            \put(-18,60){\small{29.61}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_f0_envmap_under.png}
            \put(-22,60){\small{33.49}}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % F0 OVER NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{$\mathit{F_0}\uparrow$}}} & 
        % 25.25	33.52	33.52	33.55	31.91	33.56
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_f0_noise_over.png}
            \put(-18,60){\small{25.25}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_f0_albedo_over.png}
            \put(-18,60){\small{33.52}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_f0_roughness_over.png}
            \put(-18,60){\small{33.52}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_f0_f0_over.png}
            \put(-18,60){\small{33.55}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_f0_density_over.png}
            \put(-18,60){\small{31.91}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet_over/helmet_f0_envmap_over.png}
            \put(-22,60){\small{33.56}}
        \end{subfigure}\\
        \vspace{-0.5cm}

        % DENSITY NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Density}}} & 
        % 26.18	27.33	27.33	27.33	31.84	27.4
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_density_noise.png}
            \put(-18,60){\small{26.18}}
        \end{subfigure} &        
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_density_albedo.png}
            \put(-18,60){\small{27.33}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_density_roughness.png}
            \put(-18,60){\small{27.33}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_density_f0.png}
            \put(-18,60){\small{27.33}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_density_density.png}
            \put(-18,60){\small{31.84}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_density_envmap.png}
            \put(-22,60){\small{27.40}}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % ENVMAP NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Env. Map}}} & 
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_envmap_noise.png}
            \put(-18,60){\small{26.22}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_envmap_albedo.png}
            \put(-18,60){\small{26.43}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_envmap_roughness.png}
            \put(-18,60){\small{26.43}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_envmap_f0.png}
            \put(-18,60){\small{26.42}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_envmap_density.png}
            \put(-18,60){\small{26.38}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_envmap_envmap.png}
            \put(-22,60){\small{33.60}}
        \end{subfigure}\\[0.3cm]
        \hline \\[-0.4cm]
        
        % LEARNT PARAMS
        \multicolumn{2}{c}{Original Properties}
        \put(-75,-10){\small{PSNR $\rightarrow$ 33.63}} &
        \begin{subfigure}[c]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[c]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[c]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_f0.png}
        \end{subfigure} &
        \begin{subfigure}[c]{0.13\textwidth}
            \centering
            \includegraphics[trim=50 0 0 50,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_density.png}
        \end{subfigure} &
        \begin{subfigure}[c]{0.13\textwidth}
            \centering
            \includegraphics[trim=0 -100 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftAppsMLPs_helmet/helmet_envmap.png}
        \end{subfigure}
    \end{tabular}
    % \vspace{1cm}
    \caption{Effect of manipulating one scene property before fine-tuning another for the helmet scene of the shiny-blender dataset \cite{verbin2022refnerf}. The arrows $\downarrow, \uparrow$ next to albedo, roughness, and $F_0$ denote underestimation or overestimation respectively. The bottom row contains the original properties before adding noise and fine-tuning. For every experiment, we also include the PSNR at the top right corner of the corresponding image.}
    \label{fig:finetune-image-grid-helmet}
\end{figure*}


==> sec/figures_backup.tex <==

% Illumination experiment
\begin{comment}
\begin{figure*}[h]
    \centering
    \begin{tabular}{c c c c}
        & Illumination \#1 & Illumination \#2 & Illumination \#3 \\
        % GT ENVMAP
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{GT Envmap}}} & 
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp2/envmap_forest.png}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp2/envmap_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp2/envmap_factory.png}
        \end{subfigure} \\        
        % ENVMAP
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Envmap}}} & 
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[width=\textwidth]{figures/exp2/helmet_envmap_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[width=\textwidth]{figures/exp2/helmet_envmap_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[width=\textwidth]{figures/exp2/helmet_envmap_factory.png}
        \end{subfigure} \\
        % COLOR
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Color}}} & 
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_color_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_color_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_color_factory.png}
        \end{subfigure} \\
        % ALBEDO
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Albedo}}} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_albedo_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_albedo_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_albedo_factory.png}
        \end{subfigure} \\     
        % ROUGHNESS
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Roughness}}} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_roughness_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_roughness_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_roughness_factory.png}
        \end{subfigure} \\     
        % F0
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{$\mathit{f}_0$}}} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_f0_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_f0_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_f0_factory.png}
        \end{subfigure} \\     
        % NORMALS
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Normals}}} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_world_normal_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_world_normal_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-200 80 -200 120,clip,width=\textwidth]{figures/exp2/helmet_world_normal_factory.png}
        \end{subfigure}    
    \end{tabular}
    \caption{Estimated scene properties of the helmet scene from the shiny-blender dataset under different illuminations. Due to the underconstrained nature of the problem, inverse rendering methods, NMF in this case, are biased towards reconstruction and thus fail to learn consistent scene properties.}
    \label{fig:grid_of_figures}
\end{figure*}
\end{comment}

% FINETUNING IMAGE GRID
% Separated features but same tensorf and fine-tuning only MLPs
\begin{comment}
\begin{figure*}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{c c c | c c c c c}
        & Learned Property & Manip. Property & Fin. Albedo & Fin. Roughness & Fin. $\mathit{F_0}$ & Fin. Density & Fin. Env. Map \\
        \vspace{-0.5cm}
        % ALBEDO NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Albedo}}} & 
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_albedo_noise.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_albedo_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_albedo_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_albedo_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_albedo_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b/car_albedo_envmap.png}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % ROUGHNESS NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Roughness}}} & 
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_roughness_noise.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_roughness_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_roughness_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_roughness_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_roughness_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b/car_roughness_envmap.png}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % F0 NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{$\mathit{F_0}$}}} & 
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_f0_noise.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_f0_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_f0_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_f0_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_f0_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b/car_f0_envmap.png}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % DENSITY NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Density}}} & 
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_density_noise.png}
        \end{subfigure} &        
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_density_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_density_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_density_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_density_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b/car_density_envmap.png}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % ENVMAP NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Env. Map}}} & 
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b/car_envmap.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b/car_envmap_noise.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_envmap_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_envmap_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_envmap_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b/car_envmap_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b/car_envmap_envmap.png}
        \end{subfigure}\\
    \end{tabular}
    \vspace{0.4cm}
    \caption{Effect of manipulating one scene property before finetuning another. TensoRF appearance features are split evenly among the MLPs. Only the MLPs are fine-tuned, while the input appearance features are frozen. \textbf{TO BE REMOVED}}
    \label{fig:finetune-image-grid}
\end{figure*}
\end{comment}


% FINETUNING IMAGE GRID
% Separated features with separate tensorfs and fine-tuning only MLPs
\begin{comment}
\begin{figure*}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{c c c | c c c c c}
        & Learned Property & Manip. Property & Fin. Albedo & Fin. Roughness & Fin. $\mathit{F_0}$ & Fin. Density & Fin. Env. Map \\
        \vspace{-0.5cm}
        % ALBEDO NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Albedo}}} & 
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_albedo_noise.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_albedo_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_albedo_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_albedo_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_albedo_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_albedo_envmap.png}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % ROUGHNESS NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Roughness}}} & 
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_roughness_noise.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_roughness_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_roughness_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_roughness_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_roughness_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_roughness_envmap.png}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % F0 NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{$\mathit{F_0}$}}} & 
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_f0_noise.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_f0_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_f0_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_f0_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_f0_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_f0_envmap.png}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % DENSITY NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Density}}} & 
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_density_noise.png}
        \end{subfigure} &        
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_density_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_density_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_density_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_density_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_density_envmap.png}
        \end{subfigure}\\
        \vspace{-0.5cm}
        
        % ENVMAP NOISE
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Env. Map}}} & 
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_envmap.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_envmap_noise.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_envmap_albedo.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_envmap_roughness.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_envmap_f0.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_envmap_density.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\textwidth}
            \centering
            \includegraphics[trim=0 -250 0 0,clip,width=\textwidth]{figures/exp1b_sepRFs_ftMLPs/car_envmap_envmap.png}
        \end{subfigure}\\
    \end{tabular}
    \vspace{0.4cm}
    \caption{Effect of manipulating one scene property before finetuning another. Appearance features are produced from multiple TensoRFs and each feature vector is used as input to only one of the MLPs, thus ensuring disentangled optimization of each MLP. In this case, only the MLPs are finetuned and not their input features. \textbf{TO BE REMOVED}}
    \label{fig:finetune-image-grid}
\end{figure*}
\end{comment}


 
% \begin{figure}[h]
%     \centering
%     % ALBEDO
%     \begin{subfigure}[b]{\linewidth}
%         % \raisebox{-0.2cm}{
%         \includegraphics[trim=-100 120 -180 180,clip,width=.24\linewidth]{figures/exp1/car_albedo.png}%}$\rightarrow$%
%         \raisebox{0.3cm}{$\Rightarrow$}%
%         \includegraphics[trim=-100 120 -180 180,clip,width=.24\linewidth]{figures/exp1/car_albedo_noise.png}%
%         \includegraphics[trim=-100 80 -180 120,clip,width=.24\linewidth]{figures/exp1/helmet_albedo.png}%
%         \raisebox{0.3cm}{$\Rightarrow$}%
%         \includegraphics[trim=-100 80 -180 120,clip,width=.24\linewidth]{figures/exp1/helmet_albedo_noise.png}
%         \caption{Original and manipulated albedo.}
%     \end{subfigure}\\
%     % ROUGHNESS
%     \begin{subfigure}[b]{\linewidth}
%         \includegraphics[trim=-100 120 -180 180,clip,width=.24\linewidth]{figures/exp1/car_roughness.png}%
%         \raisebox{0.3cm}{$\Rightarrow$}%
%         \includegraphics[trim=-100 120 -180 180,clip,width=.24\linewidth]{figures/exp1/car_roughness_noise.png}%
%         \includegraphics[trim=-100 80 -180 120,clip,width=.24\linewidth]{figures/exp1/helmet_roughness.png}%
%         \raisebox{0.3cm}{$\Rightarrow$}%
%         \includegraphics[trim=-100 80 -180 120,clip,width=.24\linewidth]{figures/exp1/helmet_roughness_noise.png}%
%         \caption{Original and manipulated roughness.}
%     \end{subfigure}\\
%     % F0
%     \begin{subfigure}[b]{\linewidth}
%         \includegraphics[trim=-100 120 -180 180,clip,width=.24\linewidth]{figures/exp1/car_f0.png}%
%         \raisebox{0.3cm}{$\Rightarrow$}%
%         \includegraphics[trim=-100 120 -180 180,clip,width=.24\linewidth]{figures/exp1/car_f0_noise.png}%
%         \includegraphics[trim=-100 80 -180 120,clip,width=.24\linewidth]{figures/exp1/helmet_f0.png}%
%         \raisebox{0.3cm}{$\Rightarrow$}%
%         \includegraphics[trim=-100 80 -180 120,clip,width=.24\linewidth]{figures/exp1/helmet_f0_noise.png}        
%         \caption{Original and manipulated $\mathit{F_0}$.}
%     \end{subfigure}\\
%     % NORMALS
%     \begin{subfigure}[b]{\linewidth}
%         \includegraphics[trim=-100 120 -180 180,clip,width=.24\linewidth]{figures/exp1/car_density.png}%
%         \raisebox{0.3cm}{$\Rightarrow$}%
%         \includegraphics[trim=-100 120 -180 180,clip,width=.24\linewidth]{figures/exp1/car_density_noise.png}%
%         \includegraphics[trim=-100 80 -180 120,clip,width=.24\linewidth]{figures/exp1/helmet_density.png}%
%         \raisebox{0.3cm}{$\Rightarrow$}%
%         \includegraphics[trim=-100 80 -180 120,clip,width=.24\linewidth]{figures/exp1/helmet_density_noise.png}%
%         \caption{Surface normals before and after density perturbations.}
%     \end{subfigure}\\
%     % ENVMAPS
%     \begin{subfigure}[b]{\linewidth}
%         \includegraphics[width=.22\linewidth]{figures/exp1/car_envmap.png}
%         \raisebox{0.3cm}{$\Rightarrow$}%
%         \includegraphics[width=.22\linewidth]{figures/exp1/car_envmap_noise.png}\hfill
%         \includegraphics[width=.22\linewidth]{figures/exp1/helmet_envmap.png}%
%         \raisebox{0.3cm}{$\Rightarrow$}%
%         \includegraphics[width=.22\linewidth]{figures/exp1/helmet_envmap_noise.png}%
%         \caption{Original and blurred environment maps.}
%     \end{subfigure}\\
%     \caption{Effect of adding noise on learned scene properties for the car and helmet scenes. The left figures of every pair show the original properties while the right figures show the same properties after applying noise.}
%     \label{fig:noises}
% \end{figure}


==> sec/tables_backup.tex <==

\begin{comment}
\begin{figure*}[h]
    \centering
    \begin{tabular}{c c c c}
        & Illumination \#1 & Illumination \#2 & Illumination \#3 \\
        % GT ENVMAP
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{GT Envmap}}} & 
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp2/envmap_forest.png}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp2/envmap_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/exp2/envmap_factory.png}
        \end{subfigure} \\        
        % ENVMAP
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Envmap}}} & 
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[width=\textwidth]{figures/exp2/car_envmap_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[width=\textwidth]{figures/exp2/car_envmap_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[width=\textwidth]{figures/exp2/car_envmap_factory.png}
        \end{subfigure} \\
        % COLOR
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Color}}} & 
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_color_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_color_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_color_factory.png}
        \end{subfigure} \\
        % ALBEDO
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Albedo}}} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_albedo_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_albedo_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_albedo_factory.png}
        \end{subfigure} \\     
        % ROUGHNESS
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Roughness}}} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_roughness_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_roughness_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_roughness_factory.png}
        \end{subfigure} \\     
        % F0
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{$\mathit{f}_0$}}} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_f0_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_f0_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_f0_factory.png}
        \end{subfigure} \\     
        % NORMALS
        \multirow{-6.5}{*}{{\rotatebox[origin=c]{90}{Normals}}} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_world_normal_forest.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_world_normal_christmas.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.3\textwidth}
            \includegraphics[trim=-100 120 -180 180,clip,width=\textwidth]{figures/exp2/car_world_normal_factory.png}
        \end{subfigure}
    \end{tabular}
    \caption{Estimated scene properties of the car scene from the shiny-blender dataset under different illuminations. Due to the underconstrained nature of the problem, inverse rendering methods, NMF in this case, are biased towards reconstruction and thus fail to learn consistent scene properties.}
    \label{fig:grid_of_figures}
\end{figure*}
\end{comment}

\begin{comment}
\begin{table*}[h]
    \centering
    \caption{Interplay between parameters to compensate for artificial perturbations. The compensation after finetuning a single parameter at a time is evaluated via PSNR, SSIM, LPIPS, MAE, and EPSNR. The parameter in each row corresponds to the manipulated parameter and the parameters in the columns correspond to the individually finetuned parameters while the rest remain frozen. The first column per scene corresponds to the performance with the manipulated parameter without finetuning.}
    \label{tab:compensation}
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{c c | c c c c c c | c c c c c c}
    % PSNR
    \hline
    & & \multicolumn{6}{c|}{\textbf{car}} & \multicolumn{5}{c} {\textbf{helmet}}\\
    & Parameter & - & Albedo & Rough. & $\mathbf\mathit{f}_0$ & Density & Envmap & - & Albedo & Rough. & $\mathbf\mathit{f}_0$ & Density & Envmap \\ \hline\hline
    \multirow{5}{*}{\rotatebox[origin=c]{90}{PSNR}} 
    & Albedo & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & Rough. & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & $\mathbf\mathit{f}_0$ & - & - & - & - & - & -  & - & - & - & - & - & - \\
    & Density & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & Envmap & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    % SSIM
    \hline
    \multirow{5}{*}{\rotatebox[origin=c]{90}{SSIM}} 
    & Albedo & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & Rough. & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & $\mathbf\mathit{f}_0$ & - & - & - & - & - & -  & - & - & - & - & - & - \\
    & Density & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & Envmap & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    % LPIPS
    \hline
    \multirow{5}{*}{\rotatebox[origin=c]{90}{LPIPS}} 
    & Albedo & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & Rough. & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & $\mathbf\mathit{f}_0$ & - & - & - & - & - & -  & - & - & - & - & - & - \\
    & Density & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & Envmap & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    % MAE
    \hline
    \multirow{5}{*}{\rotatebox[origin=c]{90}{MAE}} 
    & Albedo & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & Rough. & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & $\mathbf\mathit{f}_0$ & - & - & - & - & - & -  & - & - & - & - & - & - \\
    & Density & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & Envmap & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    % ePSNR
    \hline
    \multirow{5}{*}{\rotatebox[origin=c]{90}{EPSNR}} 
    & Albedo & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & Rough. & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & $\mathbf\mathit{f}_0$ & - & - & - & - & - & -  & - & - & - & - & - & - \\
    & Density & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    & Envmap & - & - & - & - & - & -  & - & - & - & - & - & - \\ 
    \hline
    \end{tabular}
\end{table*}
\end{comment}

